The case for shifting the Renyi Entropy

We introduce a variant of the R\'enyi entropy definition that aligns it with the well-known H\"older mean: in the new formulation, the r-th order R\'enyi Entropy is the logarithm of the inverse of the r-th order H\"older mean. This brings about new insights into the relationship of the R\'enyi entropy to quantities close to it, like the information potential and the partition function of statistical mechanics. We also provide expressions that allow us to calculate the R\'enyi entropies from the Shannon cross-entropy and the escort probabilities. Finally, we discuss why shifting the R\'enyi entropy is fruitful in some applications.

==> maxplus_minplus.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%
%%%% The following should be sent to a MAXPLUS/MINPLUS .sty
%%%%
%%%%    WARNING! This should be part of the TeX PRELUDE!!!
%%%%  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Algebraic operators for maxplus and minplus
%% Use the Moreau calculus rules for maxplus and minplus.
%% The following is a recipe from accents.tex for dealing with problems with \vec... IT works!
\RequirePackage{amsmath}
\let\vec\relax
\DeclareMathAccent{\vec}{\mathord}{letters}{"7E}
\RequirePackage{accents}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% UPPER GENERIC OPERATORS
% 0.- In this option the dots look TOO SMALL (REVIEWER'S REJECT)
%\DeclareMathOperator  \otimesu {\overset{\cdot}{\otimes}}%otimes upper
%\DeclareMathOperator  \oplusu {\overset{\cdot}{\oplus}}%otimes upper
% 1.- In this option the dots look alright.
\DeclareMathOperator  \otimesu {\overset{\centerdot}{\otimes}}%otimes upper
\DeclareMathOperator  \oplusu {\overset{\centerdot}{\oplus}}%otimes upper
\DeclareMathOperator  \odotu {\overset{\centerdot}{\odot}}%odot upper
\DeclareMathOperator  \oconvu {\overset{\centerdot}{\circledast}}%odot upper
% 2. In this option the dots look TOO BIG
%\DeclareMathOperator  \otimesu {\overset{\bullet}{\otimes}}%otimes upper
%\DeclareMathOperator  \oplusu {\overset{\bullet}{\oplus}}%otimes upper
%\DeclareMathOperator  \otimesu {\accentset{.}{\otimes}}%otimes upper
%\DeclareMathOperator  \otimesu {\overset{.}{\otimes}}%otimes upper
%%% The recipe for the next operator is from page 501. It doesn't work as a limit!
%%The following is the opposite bigoplus operator.
%% FVA: TODO. Change to {accents} notation.
\DeclareMathOperator*\opbigoplus{\underaccent{t \in T}{\stackrel{op}{\bigoplus}}}
%\DeclareMathOperator*\bigoplusl{\underset{\centerdot}{{\bigoplus}}}
%\DeclareMathOperator*\bigoplusl{\underset{\centerdot}{{\bigoplus}}}
\DeclareMathOperator*\bigoplusl{\sideset{}{_{\bullet}}\sum}
%\DeclareMathOperator*  \bigoplusu {\overset{\cdot}{\bigoplus}}%bigotimes upper
%\DeclareMathOperator*\bigoplusu{\overset{\centerdot}{{\bigoplus}}}
%\DeclareMathOperator*\bigoplusu{{\sum}^{\centerdot}}
\DeclareMathOperator*\bigoplusu{\sideset{}{^{\bullet}}\sum}
%\DeclareMathOperator*\bigoplusu{\protect{\sideset{}{^\centerdot}\Sigma}}
%The dec. above doesn'tw work because the limits are wrong!

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% LOWER GENERIC OPERATORS 
% 4.- In the next option the cdots are TOO SMALL (REJECTED BY REVIEWER'S)
%\DeclareMathOperator  \otimesl {\underaccent{\cdot}{\otimes}}%otimes lower
%\DeclareMathOperator  \oplusl {\underaccent{\cdot}{\oplus}}%otimes lower
% 1.- In the next option the centerdots are too LOW
%\DeclareMathOperator  \otimesl {\underset{\centerdot}{\otimes}}%otimes lower
%\DeclareMathOperator  \oplusl {\underset{\centerdot}{\oplus}}%otimes lower
% 2.- In the next option the centerdots are a BIT TOO SMALL
%\DeclareMathOperator  \otimesl {\underaccent{\centerdot}{\otimes}}%otimes lower
%\DeclareMathOperator  \oplusl {\underaccent{\centerdot}{\oplus}}%otimes lower
% 3.- In the next option the centerdots are too SMALL. BEST SO FAR
\DeclareMathOperator  \otimesl {\underaccent{\centerdot}{\otimes}}%otimes lower
\DeclareMathOperator  \oplusl {\underaccent{\centerdot}{\oplus}}%otimes lower
\DeclareMathOperator  \odotl {\underaccent{\centerdot}{\odot}}%odot lower
\DeclareMathOperator  \oconvl {\underaccent{\centerdot}{\circledast}}%odot upper
%5.-  In the next option the bullets are TOO BIG
%\DeclareMathOperator  \otimesl {\underaccent{\bullet}{\otimes}}%otimes lower
%\DeclareMathOperator  \oplusl {\underaccent{\bullet}{\oplus}}%otimes lower
%\DeclareMathOperator  \otimesl {\underaccent{\dot}{\otimes}}%otimes lower

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% LOWER  and UPPER OPERATORS on \mathbb R
\DeclareMathOperator  \plusu {\overset{\centerdot}{+}}%plus upper
\DeclareMathOperator  \timesu {\overset{\centerdot}{\times}}%times upper
\DeclareMathOperator  \minusu {\overset{\centerdot}{--}}%plus upper
\DeclareMathOperator  \plusl {\underaccent{\centerdot}{+}}%plus lower
\DeclareMathOperator  \timesl {\underaccent{\centerdot}{\times}}%times lower
\DeclareMathOperator  \minusl {\underaccent{\centerdot}{--}}%plus upper

%% Perhaps these should be operators
\DeclareMathOperator\mpunder{\backslash}%otimes lower
%\newcommand\mpunder{\ensuremath{\backslash}}
\DeclareMathOperator\mpover{\slash}%otimes lower
%\newcommand\mpover{\ensuremath{\slash}}
%%%% LOWER RESIDUATION OPERATORS
%\DeclareMathOperator\mpunderl{\underaccent{\cdot}{\backslash}}%otimes lower
%\DeclareMathOperator\mpunderl{\underaccent{\centerdot}{\backslash}}%otimes lower
\DeclareMathOperator\mpunderl{\underaccent{\;\;\;\centerdot}{\backslash}}%otimes lower
\DeclareMathOperator\underl{\underaccent{\;\;\;\centerdot}{\backslash}}%otimes lower
%\DeclareMathOperator\mpoverl{\underaccent{\cdot}{\slash}}%otimes lower
%\DeclareMathOperator\mpoverl{\underaccent{\centerdot}{\slash}}%otimes lower
\DeclareMathOperator\mpoverl{\underaccent{\!\!\!\centerdot}{\slash}}%otimes lower
\DeclareMathOperator\overl{\underaccent{\!\!\!\centerdot}{\slash}}%otimes lower
%%%% UPPER RESIDUATION OPERATORS
%\DeclareMathOperator\mpunderu{\overset{\cdot}{\backslash}}%otimes lower
\DeclareMathOperator\mpunderu{\overset{\!\!\!\centerdot}{\backslash}}%otimes lower
\DeclareMathOperator\underu{\overset{\!\!\!\centerdot}{\backslash}}%otimes lower
%\DeclareMathOperator\mpoveru{\overset{\cdot}{\slash}}%otimes lower
\DeclareMathOperator\mpoveru{\overset{\;\;\;\centerdot}{\slash}}%otimes lower
\DeclareMathOperator\overu{\overset{\;\;\;\centerdot}{\slash}}%otimes lower

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Inf and sup convolutions: for R^n
%\DeclareMathOperator*  \supconv {\underaccent{\vee}{\circledast}}%plus lower
\DeclareMathOperator*  \supconv {\underset{\vee}{\circledast}}%plus lower
%\DeclareMathOperator*  \infconv {\underaccent{\wedge}{\circledast}}%
\DeclareMathOperator*  \infconv {\underset{\wedge}{\circledast}}%
%Min and max convolutions: for R
\DeclareMathOperator*  \maxconv {\underaccent{\max}{\circledast}}%plus lower
\DeclareMathOperator*  \minconv {\underaccent{\min}{\circledast}}%
%Name for the algebras
\newcommand{\Mmp}{max-min-plus\xspace}
\newcommand{\Maxp}{max-plus\xspace}
\newcommand{\Minp}{min-plus\xspace}

%%% Commands for Maxplus and Minplus typesetting
\newcommand\maxplus{\ensuremath{\mathbb R}_{\max,+}}
\newcommand\cmaxplus{\ensuremath{\overline{\mathbb R}}_{\max,+}}
\newcommand\minplus{\ensuremath{\mathbb R}_{\min,+}}
\newcommand\cminplus{\ensuremath{\overline{\mathbb R}}_{\min,+}}
%%% Commands for Maxtimes and Mintimes typesetting
\newcommand\maxtimes{\ensuremath{\mathbb R}_{\max,\times}}
\newcommand\cmaxtimes{\ensuremath{\overline{\mathbb R}}_{\max,\times}}
\newcommand\mintimes{\ensuremath{\mathbb R}_{\min,\times}}
\newcommand\cmintimes{\ensuremath{\overline{\mathbb R}}_{\min,\times}}
%%Completed real line
\newcommand\plustimes{\ensuremath{\overline{\mathbb R}_{+,\times}}}
\newcommand\cplustimes{\ensuremath{\mathbb R}_{+,\times}}
% Other positive semifields
\newcommand\R{\ensuremath{\mathbb R}}%just lackboard R
\newcommand\nonnegativeR{\ensuremath{\mathbb R}_0^+}%the nonnegative reals with multiplicative products
%\newcommand\nnR{\ensuremath{\mathbb R}_0^+}%An alias for the positive reals
\newcommand\nnR{\ensuremath{\mathbb R}_{\geq{0}}}%An alias for the positive reals
\newcommand\nnQ{\ensuremath{\mathbb Q}_{\geq{0}}}%An alias for the positive reals
\newcommand\nnRr[1][r]{\ensuremath{{\left (\nnR\right)_{#1}}}}%The semifields obtained by the Hölder mean transformation 
\newcommand{\hR}{\ensuremath{\mathbb H}} %Hartley semifields: simple and of order R
\newcommand\hRr[1][r]{\ensuremath{{\hR_{#1}}}}%The semifields obtained by the log-Hölder mean transformation 
\newcommand\cR{\ensuremath{{\mathbb R}_{\pm \infty}}}
%%Completed idempotent semimfield
\newcommand\cK{\ensuremath{\overline {\mathcal K}}}
\newcommand{\icK}{\ensuremath{\linv{\overline {\mathcal K}}}}
\newcommand{\dcK}{\ensuremath{\lconj{\overline {\mathcal K}}}}
%% The maxminplus or minmax algebra
%\newcommand\maxminplus{\ensuremath\overline{\mathbb R}_{\max,\min,+}}
\newcommand\maxminplus{\ensuremath\overline{\mathbb R}_{\max,\plusl}^{\min,\plusu}}
%\newcommand\maxmintimes{\ensuremath\overline{\mathbb R_0^+}_{\max,\min,\times}}
\newcommand\maxmintimes{\ensuremath\overline{\mathbb R}_{\max,\timesl}^{\min,\timesu}}
%% The positive reals and their completion
\newcommand\Rplusplustimes{\ensuremath{\mathbb R}^{+}_{+,\times}}
\newcommand\cnnRplustimes{\ensuremath{\overline{\mathbb R}}^{+}_{+,\times}}%completed nonnegative R plust times
\newcommand\Nplustimes{\ensuremath{{\mathbb N}}_{+,\times}}
\newcommand\cNplustimes{\ensuremath{\overline{\mathbb N}}_{+,\times}}

\newcommand\parmaxplus{\ensuremath{\left(\maxplus\right)}}
\newcommand\parminplus{\ensuremath{\left(\minplus \right)}}
\newcommand\parcmaxplus{\ensuremath{\left(\cmaxplus\right)}}
\newcommand\parcminplus{\ensuremath{\left(\cminplus \right)}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Different types of scalar product
%% Declaring brackets
\newcommand\bracket[2]{\ensuremath{\langle {#1}\mid{#2} \rangle}}
\newcommand\bracketdot{\ensuremath{\bracket{\cdot}{\cdot}}}
\newcommand\sqbracket[2]{\ensuremath{\left [{#1}\mid{#2} \right ]}}
\newcommand\sqbracketdot{\ensuremath{\sqbracket{\cdot}{\cdot}}}

%% Brackets with Relations in the middel
\newcommand\Rbracket[3]{\ensuremath{\langle {#1}\mid{#2}\mid{#3} \rangle}}
\newcommand\Rbracketdot[1]{\ensuremath{\Rbracket{\cdot}{#1}{\cdot}}}
\newcommand\Rsqbracket[3]{\ensuremath{\left [{#1}\mid{#2}\mid{#3} \right ]}}
\newcommand\Rsqbracketdot[1]{\ensuremath{\Rsqbracket{\cdot}{#1}{\cdot}}}

%% And ket-bras
\newcommand\ketbra[2]{\ensuremath{\rangle {#1}\mid{#2} \langle}}
\newcommand\ketbradot{\ensuremath{\ketbra{\cdot}{\cdot}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Different types of adjoints for brackets
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\RequirePackage{amssymb}
\RequirePackage{amsmath}
%\RequirePackage{galois_connections}
%left and right Galois connection adjoints (contravariant, antitone)
%\newcommand\lgc[1]{\ensuremath{#1}_\varphi^\circledast}%y_\varphi^*
%\newcommand\lgc[1]{\ensuremath{#1}_\varphi^{\_}}%y_\varphi^*
%\newcommand\lgc[1]{\ensuremath{\left( #1\right)}_\varphi^{-}}%y_\varphi^*
%Use V 2 of Galois connections adjoint functions
\newcommand\lgc[1]{\ladj{+}{\varphi}{#1}}
%\newcommand\rgc[1]{\ensuremath{}_\varphi^\circledast{#1}}%{}_\varphi^*x
%\newcommand\rgc[1]{\ensuremath{}_\varphi^{\_}{#1}}%{}_\varphi^*x
%\newcommand\rgc[1]{\ensuremath{}_\varphi^{-}{\left( #1\right)}}%{}_\varphi^*x
%\newcommand\rgc[1]{\ensuremath{}_\varphi^{-}{\left( #1\right)}}%{}_\varphi^*x
%Use V 2 of Galois connections adjoint functions
\newcommand\rgc[1]{\radj{+}{\varphi}{#1}}%{}_\varphi^*x

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% The conjugations and inversions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Left and right refer to left and right adjoints in the GC or adjunction NOT to the left and right continuous functions of the brackets.
%Right and left CGreen conjugates
%\newcommand\rconj[1]{\ensuremath{#1}^\ast}
\newcommand\lconj[1]{\ensuremath{#1}^\circledast}
%\newcommand\lconj[1]{\ensuremath{}^\ast{#1}}
\newcommand\rconj[1]{\ensuremath{\vphantom{#1}}^\circledast{#1}}
%Right and left CGQ conjugates
\newcommand\lphiconj[1]{\ensuremath{#1}_\varphi^\circledast}
\newcommand\rphiconj[1]{\ensuremath{\vphantom{#1}}_\varphi^\circledast{#1}}

%Right and left inverses
\newcommand\linv[1]{\ensuremath{#1}^{-1}}
\newcommand\rinv[1]{\ensuremath{{\vphantom{#1}}^{-1}{#1}}}
%transposes
\newcommand\transp[1]{\ensuremath{{#1}^{\textsc{t}}}}
%\newcommand\transp[1]{\ensuremath{{#1}^{\rm T}}}%too big
%\newcommand\transp[1]{\ensuremath{{#1}^{\top}}}%recalls the orthogonal adjoint

%Pseudo-inverse, aka transitive closure, and TR-closure
\newcommand\tclosure[1]{\ensuremath{{#1}^\oplus}} 
\newcommand\trclosure[1]{\ensuremath{{#1}^\circledast}}
\newcommand\tclosurel[1]{\ensuremath{{#1}^{\underaccent{\centerdot}{\oplus}}}}%otimes lower
\newcommand\trclosurel[1]{\ensuremath{{#1}^{\underaccent{\centerdot}{\circledast}}}}%otimes lower

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% The following doesn't work because sideset only applies to operators.
%\newcommand\rRgc[2]{\ensuremath\sideset{_\varphi^{#1}}{}{\left( #2\right)}}%{}_\varphi^*x
%% Commands for GGCC induced by a relation
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\rRgc[2]{\ensuremath{\left( #2\right)}_\varphi^{#1}}%y_\varphi^*
\newcommand\lRgc[2]{\ensuremath{}_\varphi^{#1}{\left( #2\right)}}%{}_\varphi^*x
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Commands for completed semirings
\newcommand{\complete}[1]{\ensuremath{\overline{#1}}}
\newcommand{\completeK}{\complete{\mathcal K}}
%%%Interesting classes of K-FCA
\RequirePackage{fca}
\newcommand{\FCAabb}{FCA\xspace}
\newcommand\RmaxFCA{$\left(\maxplus \right )$-\FCA}
\newcommand\RminFCA{$\left(\minplus \right )$-\FCA}
\newcommand\cRmaxFCA{$\left(\cmaxplus \right )$-\FCA}
\newcommand\cRminFCA{$\left(\cminplus \right )$-\FCA}
\newcommand\maxminplusFCA{$\left(\maxminplus \right )$-\FCA}
\newcommand\cRmaxFCAabb{$\left(\cmaxplus \right )$-\FCAabb}
\newcommand\cRminFCAabb{$\left(\cminplus \right )$-\FCAabb}
\newcommand\maxminplusFCAabb{$\left(\maxminplus \right )$-\FCAabb}
%\newcommand\KFCA{$\left(\mathcal K\right )$-\FCA}
\newcommand\KFCA{$\mathcal K$-\FCA}
\newcommand{\KFCAabb}{$\mathcal K$-FCA\xspace}
\newcommand\cKFCA{$\overline{\mathcal K}$-\FCA}
\newcommand\GKFCA{Generalized $\mathcal K$-\FCA}
\newcommand\GFCA{Generalized \FCA}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Some hyphenation for semimodules over semirings and order morphisms
\hyphenation{%
in-fi-mum ma-xi-mum
mo-noid mo-noids di-oids di-oid 
semi-ring semi-rings  
zero-sum-free 
mo-du-loid 
mul-ti-pli-ca-tive
semi-mo-dule semi-mo-dules bi-semi-mo-dule
para-me-ter}

%%% Local Variables: 
%%% mode: plain-tex
%%% TeX-master: t
%%% End: 

